A Thorough Study of LoRaWAN Performance Under Different Parameter Settings

LoRaWAN is an emerging Low-Power Wide Area Network (LPWAN) technology, which is gaining momentum thanks to its flexibility and ease of deployment. Conversely to other LPWAN solutions, LoRaWAN indeed permits the configuration of several network parameters that affect different network performance indexes, such as energy efficiency, fairness, and capacity, in principle making it possible to adapt the network behavior to the specific requirements of the application scenario. Unfortunately, the complex and sometimes elusive interactions among the different network components make it rather difficult to predict the actual effect of a certain parameters setting, so that flexibility can turn into a stumbling block if not deeply understood. In this paper we shed light on such complex interactions, by observing and explaining the effect of different parameters settings in some illustrative scenarios. The simulation-based analysis reveals various trade-offs and highlights some inefficiencies in the design of the LoRaWAN standard. Furthermore, we show how significant performance gains can be obtained by wisely setting the system parameters, possibly in combination with some novel network management policies.

==> img/ack_timeout/ack_timeout.tex <==
\begin{tikzpicture}

\begin{axis}[%
xlabel=Number of End devices,
ylabel=Packet success ratio,
xmin=0,
xmax=4500,
xminorgrids,
yminorgrids,
ymin=0.55,
ymax=1,
xmajorgrids,
ymajorgrids,
% yticklabel style={
    % /pgf/number format/fixed,
    % /pgf/number format/precision=2,
    % },
% xticklabel style={
    % /pgf/number format/fixed,
    % /pgf/number format/precision=5,
    % },
legend entries={
	\scriptsize{with ACK\_TIMEOUT},
  	\scriptsize{without ACK\_TIMEOUT}
	},
  legend pos=north east,
  legend style={legend cell align=left,align=left,draw=white!15!black},
  mark options={solid}
]
% with
\addplot [color=black, solid, line width=0.8pt]
table[row sep=crcr]{
1	1 \\
501	0.96721 \\
1001	0.91235 \\
1501	0.8579 \\
2001	0.80317 \\
2501	0.76084 \\
3001	0.70596 \\
3501	0.66045 \\
4001	0.62268 \\
4501	0.57804 \\
};

% without
\addplot [color=black, dashed, mark=x, line width=0.8pt]
table[row sep=crcr]{
1	1 \\
501	0.9554 \\
1001	0.90442 \\
1501	0.85967 \\
2001	0.80185 \\
2501	0.75387 \\
3001	0.7046 \\
3501	0.6551 \\
4001	0.61922 \\
4501	0.57536 \\
};

\end{axis}
\end{tikzpicture}%

==> img/ack_timeout/ack_timeout_mac.tex <==
\begin{tikzpicture}

\begin{axis}[%
xlabel=Number of End devices,
ylabel=Packet success ratio,
xmin=0,
xmax=4500,
xminorgrids,
yminorgrids,
ymin=0,
ymax=1,
xmajorgrids,
ymajorgrids,
% yticklabel style={
    % /pgf/number format/fixed,
    % /pgf/number format/precision=2,
    % },
% xticklabel style={
    % /pgf/number format/fixed,
    % /pgf/number format/precision=5,
    % },
legend entries={
	\scriptsize{with ACK\_TIMEOUT},
  	\scriptsize{without ACK\_TIMEOUT}
	},
  legend pos=north east,
  legend style={legend cell align=left,align=left,draw=white!15!black},
  mark options={solid}
]
% with
\addplot [color=black, solid, line width=0.9pt]
table[row sep=crcr]{
1	1 \\
501	0.83553 \\
1001	0.48292 \\
1501	0.33304 \\
2001	0.26102 \\
2501	0.20932 \\
3001	0.17664 \\
3501	0.15281 \\
4001	0.13902 \\
4501	0.12002 \\
};
% without
\addplot [color=black, dashed, mark=x, line width=0.8pt]
table[row sep=crcr]{
1	1 \\
501	0.82914 \\
1001	0.48971 \\
1501	0.33464 \\
2001	0.25512 \\
2501	0.2106 \\
3001	0.17504 \\
3501	0.15293 \\
4001	0.13742 \\
4501	0.12331 \\
};

\end{axis}
\end{tikzpicture}%

==> img/causesLosses/causesLosses.tex <==
\begin{tikzpicture}

\begin{axis}[%
xlabel=Number of devices ($N$),
ylabel=Packet loss probability,
xmin=0,
xmax=5500,
% xminorgrids,
% yminorgrids,
ymin=0,
ymax=1,
xmajorgrids,
ymajorgrids,
% yticklabel style={
    % /pgf/number format/fixed,
    % /pgf/number format/precision=2,
    % },
% xticklabel style={
    % /pgf/number format/fixed,
    % /pgf/number format/precision=5,
    % },
legend entries={
	\scriptsize{Total failure probability},
  	\scriptsize{Probability of interfered packets},
  	\scriptsize{Probability of no more receivers available},
  	\scriptsize{Probability of packets under sensitivity}
	},
  legend pos=north west,
  legend style={legend cell align=left,align=left,draw=white!15!black},
  mark options={solid}
]
% Total
\addplot [color=black, solid, line width=0.9pt]
table[row sep=crcr]{
1 0 \\
501 0.10502 \\
1001 0.21272 \\
1501 0.31454 \\
2001 0.40289 \\
2501 0.47768 \\
3001 0.54534 \\
3501 0.60003 \\
4001 0.64234 \\
4501 0.68405 \\
5001 0.71381 \\
5501 0.73865 \\
};
% Interfered
\addplot [color=black, solid, mark=x, line width=0.8pt]
table[row sep=crcr]{
1 0 \\
501 0.094119 \\
1001 0.16085 \\
1501 0.20558 \\
2001 0.22891 \\
2501 0.24304 \\
3001 0.25083 \\
3501 0.25168 \\
4001 0.24811 \\
4501 0.24694 \\
5001 0.23919 \\
5501 0.23475 \\
};

% No more rx
\addplot [color=black, solid, mark=o, line width=0.8pt]
table[row sep=crcr]{
1 0 \\
501 0.010905 \\
1001 0.051869 \\
1501 0.10895 \\
2001 0.17398 \\
2501 0.23463 \\
3001 0.29451 \\
3501 0.34835 \\
4001 0.39422 \\
4501 0.43712 \\
5001 0.47463 \\
5501 0.5039 \\
};

% Under sensitivity
\addplot [color=black, solid, mark=square, line width=0.8pt]
table[row sep=crcr]{
	1 0 \\
	501 0 \\
	1001 0 \\
	1501 0 \\
	2001 0 \\
	2501 0 \\
	3001 0 \\
	3501 0 \\
	4001 0 \\
	4501 0 \\
	5001 0 \\
	5501 0 \\
};

\end{axis}
\end{tikzpicture}%

==> img/contour-2.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\begin{tikzpicture}

\begin{axis}[%
% width=4.521in,
% height=3.566in,
% at={(0.758in,0.481in)},
width=0.7\linewidth,
scale only axis,
xmin=300,
xmax=2000,
xtick={500, 1000, 1500, 2000},
xlabel={\small Number of devices},
ylabel={\small \% of devices using confirmed traffic},
ylabel near ticks,
xlabel near ticks,
ymin=0,
ymax=100,
axis background/.style={fill=white}
]
\addplot[contour prepared, contour prepared format=matlab] table[row sep=crcr] {%
%
0.5	2\\
2100	97.5324829481642\\
2022.26083354429	100\\
0.55	2\\
2100	89.7060523092536\\
1775.68900388268	100\\
0.6	2\\
2100	81.8796216703429\\
1529.11717422108	100\\
0.65	3\\
2100	73.4120207334749\\
1893.99492648647	80\\
1282.54534455948	100\\
0.7	4\\
2100	64.7417636170001\\
1622.87735273571	80\\
1100	97.6267365342432\\
1038.92872676665	100\\
0.75	5\\
2100	55.7471039602024\\
1896.8440205066	60\\
1351.75977898495	80\\
1100	88.4870826224714\\
803.737687357102	100\\
0.8	5\\
2100	46.3608844947477\\
1448.47505230224	60\\
1100	78.3172402740495\\
1064.57739442426	80\\
568.546647947551	100\\
0.85	6\\
2100	35.6319045564709\\
1839.94948250768	40\\
1100	56.0910453050927\\
948.127238445294	60\\
568.462470394341	80\\
333.355608537999	100\\
0.9	5\\
2100	22.0797184759211\\
1100	37.6868135702025\\
969.60133674442	40\\
266.453757316062	60\\
100	76.283166956742\\
0.91	6\\
2100	19.0331661005681\\
2003.08850722151	20\\
1100	32.1046652804332\\
654.925154269994	40\\
130.119061090216	60\\
100	62.9463660551745\\
0.92	5\\
2100	14.8783147923093\\
1586.62313215279	20\\
1100	26.5225169906639\\
340.248971795569	40\\
100	49.8988694118867\\
0.93	4\\
2100	10.7234634840506\\
1170.15775708409	20\\
1100	20.9403687008947\\
100	35.9967164002267\\
0.94	3\\
2100	6.56861217579177\\
1100	13.3155142545932\\
100	19.4897133879348\\
0.95	3\\
2100	2.41376086753296\\
1100	5.27683211614291\\
100	10.1931819238241\\
};
\end{axis}
\end{tikzpicture}%

==> img/contour-4.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\begin{tikzpicture}

\begin{axis}[%
width=0.7\linewidth,
scale only axis,
xmin=300,
xmax=2000,
xtick={500, 1000, 1500, 2000},
xlabel={\small Number of devices},
ylabel={\small \% of devices using confirmed traffic},
ylabel near ticks,
xlabel near ticks,
ymin=0,
ymax=100,
axis background/.style={fill=white}
]
\addplot[contour prepared, contour prepared format=matlab] table[row sep=crcr] {%
%
0.55	2\\
2100	96.6501051191399\\
2011.89056275552	100\\
0.6	2\\
2100	89.2784964277184\\
1818.00140608416	100\\
0.65	2\\
2100	81.9068877362969\\
1624.11224941281	100\\
0.7	3\\
2100	73.6844795565425\\
1903.3334518306	80\\
1430.22309274145	100\\
0.75	3\\
2100	65.1651890430565\\
1638.04107044415	80\\
1236.33393607009	100\\
0.8	5\\
2100	55.521420865935\\
1938.40617086161	60\\
1372.7486890577	80\\
1100	95.5191433350038\\
1009.2014143787	100\\
0.85	5\\
2100	44.1459997383653\\
1527.96397412025	60\\
1107.45630767125	80\\
1100	80.4242568787398\\
703.323667596534	100\\
0.9	6\\
2100	28.8609362447966\\
1573.16807093285	40\\
1117.52177737889	60\\
1100	60.841527167785\\
584.8856819702	80\\
397.445920814368	100\\
0.91	6\\
2100	25.355495508654\\
1407.37513304883	40\\
1100	54.0424613333737\\
922.766070591629	60\\
478.883521646172	80\\
336.270371457935	100\\
0.92	6\\
2100	21.8500547725115\\
1241.58219516481	40\\
1100	46.4681956584309\\
697.435284998378	60\\
372.881361322145	80\\
275.094822101501	100\\
0.93	7\\
2100	17.0608493599718\\
1839.26662642265	20\\
1100	38.0332262604632\\
1059.68127138041	40\\
472.104499405129	60\\
266.879200998119	80\\
213.919272745068	100\\
0.94	7\\
2100	10.8369120972594\\
1287.13835598287	20\\
1100	24.564940705873\\
783.582328563265	40\\
246.773713811877	60\\
160.877040674092	80\\
152.743723388635	100\\
0.95	5\\
2100	4.61297483454703\\
1100	12.0886564502715\\
778.341345685983	20\\
507.483385746117	40\\
100	56.1783292865404\\
};
\end{axis}
\end{tikzpicture}%

==> img/contour-8.tex <==
% This file was created by matlab2tikz.
%
% The latest updates can be retrieved from
% http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
% where you can also make suggestions and rate matlab2tikz.
%
\begin{tikzpicture}

  \begin{axis}[%
width=0.7\linewidth,
scale only axis,
xmin=300,
xmax=2000,
xtick={500, 1000, 1500, 2000},
xlabel={\small Number of devices},
ylabel={\small \% of devices using confirmed traffic},
ylabel near ticks,
xlabel near ticks,
ymin=0,
ymax=100,
axis background/.style={fill=white}
    ]
    \addplot[contour prepared, contour prepared format=matlab] table[row sep=crcr] {%
      %
      0.6	2\\
      2100	97.7111844019015\\
      2049.7606812927	100\\
      0.65	2\\
      2100	89.7415857641716\\
      1874.8286307322	100\\
      0.7	2\\
      2100	81.7719871264417\\
      1699.89658017171	100\\
      0.75	3\\
      2100	73.4462624534554\\
      1905.58051920086	80\\
      1524.96452961121	100\\
      0.8	3\\
      2100	65.0187161756919\\
      1655.57368568074	80\\
      1350.03247905072	100\\
      0.85	4\\
      2100	53.3874092339551\\
      1910.39983750254	60\\
      1405.56685216063	80\\
      1175.10042849023	100\\
      0.9	6\\
      2100	34.5998141328603\\
      1922.56901490876	40\\
      1441.65716160685	60\\
      1155.56001864051	80\\
      1100	85.6054441672699\\
      818.564852760016	100\\
      0.91	6\\
      2100	28.63616258902\\
      1726.62454295952	40\\
      1347.90862642771	60\\
      1105.55865193649	80\\
      1100	80.5608117822433\\
      719.934726582495	100\\
      0.92	6\\
      2100	22.6725110451796\\
      1530.68007101028	40\\
      1254.16009124858	60\\
      1100	72.9826348179991\\
      931.540383077276	80\\
      621.304600404975	100\\
      0.93	7\\
      2100	16.5447506547986\\
      1894.15308217092	20\\
      1334.73559906103	40\\
      1160.41155606944	60\\
      1100	65.0875759405977\\
      742.010757701536	80\\
      522.674474227456	100\\
      0.94	7\\
      2100	10.2837286473062\\
      1521.15190224385	20\\
      1138.79112711179	40\\
      1100	47.1524829741497\\
      862.022673430338	60\\
      552.481132325794	80\\
      424.044348049935	100\\
      0.95	6\\
      2100	4.02270663981386\\
      1148.15072231679	20\\
      1100	22.7727897585705\\
      763.661258329522	40\\
      362.951506950052	80\\
      325.414221872415	100\\
    };
  \end{axis}
\end{tikzpicture}%

==> img/histogram.tex <==
\begin{tikzpicture}
  \usetikzlibrary{patterns}
  \begin{axis}[
    ybar stacked,
    % enlargelimits=0.15,
    bar width=0.6cm,
    ylabel={Probability},
    symbolic x coords={1 tx, 2 tx, 4 tx, 8 tx,
      4 tx + ADR, 8 tx + ADR},
    xtick=data,
    x tick label style={rotate=45,anchor=east},
    legend pos=south west,
    legend style={legend cell align=left,align=left,draw=white!15!black,
      at={(0.5,1.2)},	anchor=north, legend columns=2},
    mark options={solid}
    ]
    \addplot+[black, ybar, pattern=crosshatch] plot coordinates
    {
      (1 tx, 0.8554)
      (2 tx, 0.7256)
      (4 tx, 0.5153)
      (8 tx, 0.2859)
      (4 tx + ADR, 0.0542)
      (8 tx + ADR, 0.0065)
    };
    \addplot+[black, ybar, pattern=north west lines] plot coordinates
    {
      (1 tx, 0.1188)
      (2 tx, 0.1855)
      (4 tx, 0.2417)
      (8 tx, 0.2386)
      (4 tx + ADR, 0.4024)
      (8 tx + ADR, 0.2427)
    };
    \addplot+[black, ybar, pattern=dots] plot coordinates
    {
      (1 tx, 0.0258)
      (2 tx, 0.0889)
      (4 tx, 0.2430)
      (8 tx, 0.4756)
      (4 tx + ADR, 0.5434)
      (8 tx + ADR, 0.7507)
    };
    \legend{Received, Interfered, Receiver saturation}
  \end{axis}
\end{tikzpicture}

==> img/model/model.tex <==
\begin{tikzpicture}

\begin{axis}[%
xlabel=Network packet arrival rate,
ylabel=Packet success ratio,
xmin=1e-2,
xmax=1e1,
xmode=log,
xminorgrids,
yminorgrids,
ymin=0,
ymax=1,
ymajorgrids,
% yticklabel style={
    % /pgf/number format/fixed,
    % /pgf/number format/precision=2,
    % },
% xticklabel style={
    % /pgf/number format/fixed,
    % /pgf/number format/precision=5,
    % },
legend entries={\scriptsize{Simulator, Duty Cycle on},
  \scriptsize{Simulator, Duty Cycle off},
	\scriptsize{Model}
	},
  legend pos=south west,
  legend style={legend cell align=left,align=left,draw=white!15!black},
  mark options={solid}
]
\addplot [color=black, solid, mark=o, line width=0.8pt]
table[row sep=crcr]{
  10                0.0161 \\
  3.33333333333     0.04255 \\
  1                 0.1287 \\
  0.333333333333    0.31235 \\
  0.111111111111    0.60595 \\
  0.037037037037    0.8516 \\
  0.0123456790123   0.965 \\
  0.00411522633745  0.9918 \\
  0.00137174211248  0.99835 \\
};
\addplot [color=black, solid, mark=x, line width=0.8pt]
table[row sep=crcr]{
 10 0.0993 \\
 3.33333333333 0.2684 \\
 1 0.53555 \\
 0.333333333333 0.76285 \\
 0.111111111111 0.90735 \\
 0.037037037037 0.96755 \\
 0.0123456790123 0.9892 \\
 0.00411522633745 0.99575 \\
 0.00137174211248 0.9989 \\
};

\addplot [color=black, dashed, line width=0.8pt]
table[row sep=crcr]{
  0.0100   0.9985 \\
  0.0144   0.9978 \\
  0.0207   0.9968 \\
  0.0298   0.9954 \\
  0.0428   0.9934 \\
  0.0616   0.9905 \\
  0.0886   0.9863 \\
  0.1274   0.9802 \\
  0.1833   0.9715 \\
  0.2637   0.9589 \\
  0.3793   0.9409 \\
  0.5456   0.9154 \\
  0.7848   0.8802 \\
  1.1288   0.8330 \\
  1.6238   0.7728 \\
  2.3357   0.7005 \\
  3.3598   0.6193 \\
  4.8329   0.5345 \\
  6.9519   0.4513 \\
  10.0000  0.3736 \\
};

\end{axis}
\end{tikzpicture}%
